Categorical Models for a Semantically Linear Lambda-calculus

This paper is about a categorical approach to model a very simple Semantically Linear lambda calculus, named Sll-calculus. This is a core calculus underlying the programming language SlPCF. In particular, in this work, we introduce the notion of Sll-Category, which is able to describe a very large class of sound models of Sll-calculus. Sll-Category extends in the natural way Benton, Bierman, Hyland and de Paiva's Linear Category, in order to soundly interpret all the constructs of Sll-calculus. This category is general enough to catch interesting models in Scott Domains and Coherence Spaces.

==> eptcsdata.tex <==
\providecommand{\event}{M. Florido and I. Mackie (Eds.): First International\\
Workshop on Linearity (LINEARITY 2009)}
\providecommand{\volume}{22}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{1}
\providecommand{\eid}{1}

